A Herglotz-based integrator for nonholonomic mechanical systems

We propose a numerical scheme for the time-integration of nonholonomic mechanical systems, both conservative and nonconservative. The scheme is obtained by simultaneously discretizing the constraint equations and the Herglotz variational principle. We validate the method using numerical simulations and contrast them against the results of standard methods from the literature.

==> Article-NonHolonomic(corrected)ARXIV_with_fig/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamthm{example}{Example}

% Sets running headers as well as PDF title and authors
\headers{Nonholonomic Herglotz Integrator}{E. Maciel, I. Ortiz, and C. E. Schaerer}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A Herglotz-based integrator for nonholonomic mechanical systems}



%\title{Contact Integrator for nonholonomic systems\thanks{Submitted to the editors DATE.
%\funding{This work was funded by ...}}}

% Authors: full names plus addresses.
% \author{Elias Maciel\thanks{FPUNA 
%   (\email{emaciel@pol.una.py}, %\url{http://www.imag.com/\string~ddoe/}
%   ).}
% \and Inocencio Ortiz\thanks{FPUNA 
%   (\email{iortiz@pol.una.py}, %\email{jesmith@fictional.edu}
%   ).}
% \and Christian E. Schaerer\footnotemark[3]}

% \usepackage{amsopn}
% \DeclareMathOperator{\diag}{diag}

%Modificación para JGM
\author{Elias Maciel\and Inocencio Ortiz\and Christian E. Schaerer}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

